AI-assisted Agile Propagation Modeling for Real-time Digital Twin Wireless Networks

Accurate channel modeling in real-time faces remarkable challenge due to the complexities of traditional methods such as ray tracing and field measurements. AI-based techniques have emerged to address these limitations, offering rapid, precise predictions of channel properties through ground truth data. This paper introduces an innovative approach to real-time, high-fidelity propagation modeling through advanced deep learning. Our model integrates 3D geographical data and rough propagation estimates to generate precise path gain predictions. By positioning the transmitter centrally, we simplify the model and enhance its computational efficiency, making it amenable to larger scenarios. Our approach achieves a normalized Root Mean Squared Error of less than 0.035 dB over a 37,210 square meter area, processing in just 46 ms on a GPU and 183 ms on a CPU. This performance significantly surpasses traditional high-fidelity ray tracing methods, which require approximately three orders of magnitude more time. Additionally, the model's adaptability to real-world data highlights its potential to revolutionize wireless network design and optimization, through enabling real-time creation of adaptive digital twins of real-world wireless scenarios in dynamic environments.

==> figures/ecdf_data.tex <==
% Data for NU Campus (DL)
\addplot+[mark=none] coordinates {%
(0.0196,0.0033) (0.0203,0.0067) (0.0203,0.0100) (0.0204,0.0134) (0.0207,0.0167) (0.0208,0.0201) (0.0208,0.0234) (0.0210,0.0268) (0.0212,0.0301) (0.0213,0.0334) (0.0213,0.0368) (0.0214,0.0401) (0.0217,0.0435) (0.0219,0.0468) (0.0221,0.0502) (0.0221,0.0535) (0.0221,0.0569) (0.0221,0.0602) (0.0221,0.0635) (0.0222,0.0669) (0.0222,0.0702) (0.0223,0.0736) (0.0224,0.0769) (0.0225,0.0803) (0.0225,0.0836) (0.0225,0.0870) (0.0226,0.0903) (0.0227,0.0936) (0.0228,0.0970) (0.0228,0.1003) (0.0229,0.1037) (0.0229,0.1070) (0.0229,0.1104) (0.0230,0.1137) (0.0231,0.1171) (0.0231,0.1204) (0.0231,0.1237) (0.0232,0.1271) (0.0232,0.1304) (0.0233,0.1338) (0.0233,0.1371) (0.0234,0.1405) (0.0234,0.1438) (0.0235,0.1472) (0.0235,0.1505) (0.0235,0.1538) (0.0236,0.1572) (0.0236,0.1605) (0.0236,0.1639) (0.0237,0.1672) (0.0237,0.1706) (0.0237,0.1739) (0.0237,0.1773) (0.0238,0.1806) (0.0238,0.1839) (0.0239,0.1873) (0.0239,0.1906) (0.0240,0.1940) (0.0240,0.1973) (0.0240,0.2007) (0.0241,0.2040) (0.0241,0.2074) (0.0242,0.2107) (0.0242,0.2140) (0.0242,0.2174) (0.0242,0.2207) (0.0242,0.2241) (0.0243,0.2274) (0.0243,0.2308) (0.0244,0.2341) (0.0244,0.2375) (0.0244,0.2408) (0.0245,0.2441) (0.0245,0.2475) (0.0245,0.2508) (0.0245,0.2542) (0.0245,0.2575) (0.0246,0.2609) (0.0246,0.2642) (0.0246,0.2676) (0.0247,0.2709) (0.0247,0.2742) (0.0247,0.2776) (0.0247,0.2809) (0.0248,0.2843) (0.0248,0.2876) (0.0248,0.2910) (0.0249,0.2943) (0.0249,0.2977) (0.0249,0.3010) (0.0249,0.3043) (0.0250,0.3077) (0.0250,0.3110) (0.0250,0.3144) (0.0250,0.3177) (0.0251,0.3211) (0.0251,0.3244) (0.0251,0.3278) (0.0251,0.3311) (0.0252,0.3344) (0.0252,0.3378) (0.0253,0.3411) (0.0253,0.3445) (0.0254,0.3478) (0.0254,0.3512) (0.0255,0.3545) (0.0255,0.3579) (0.0255,0.3612) (0.0256,0.3645) (0.0256,0.3679) (0.0256,0.3712) (0.0256,0.3746) (0.0257,0.3779) (0.0257,0.3813) (0.0257,0.3846) (0.0257,0.3880) (0.0258,0.3913) (0.0258,0.3946) (0.0258,0.3980) (0.0258,0.4013) (0.0258,0.4047) (0.0258,0.4080) (0.0258,0.4114) (0.0258,0.4147) (0.0258,0.4181) (0.0259,0.4214) (0.0259,0.4247) (0.0259,0.4281) (0.0259,0.4314) (0.0260,0.4348) (0.0260,0.4381) (0.0261,0.4415) (0.0261,0.4448) (0.0261,0.4482) (0.0262,0.4515) (0.0263,0.4548) (0.0264,0.4582) (0.0264,0.4615) (0.0264,0.4649) (0.0265,0.4682) (0.0265,0.4716) (0.0266,0.4749) (0.0266,0.4783) (0.0267,0.4816) (0.0267,0.4849) (0.0267,0.4883) (0.0267,0.4916) (0.0267,0.4950) (0.0268,0.4983) (0.0268,0.5017) (0.0268,0.5050) (0.0269,0.5084) (0.0269,0.5117) (0.0270,0.5151) (0.0271,0.5184) (0.0271,0.5217) (0.0272,0.5251) (0.0272,0.5284) (0.0272,0.5318) (0.0272,0.5351) (0.0272,0.5385) (0.0272,0.5418) (0.0274,0.5452) (0.0274,0.5485) (0.0274,0.5518) (0.0275,0.5552) (0.0275,0.5585) (0.0275,0.5619) (0.0275,0.5652) (0.0276,0.5686) (0.0276,0.5719) (0.0276,0.5753) (0.0277,0.5786) (0.0277,0.5819) (0.0277,0.5853) (0.0278,0.5886) (0.0278,0.5920) (0.0278,0.5953) (0.0284,0.5987) (0.0285,0.6020) (0.0285,0.6054) (0.0285,0.6087) (0.0285,0.6120) (0.0286,0.6154) (0.0286,0.6187) (0.0287,0.6221) (0.0289,0.6254) (0.0290,0.6288) (0.0291,0.6321) (0.0292,0.6355) (0.0292,0.6388) (0.0293,0.6421) (0.0293,0.6455) (0.0294,0.6488) (0.0294,0.6522) (0.0296,0.6555) (0.0296,0.6589) (0.0297,0.6622) (0.0297,0.6656) (0.0299,0.6689) (0.0299,0.6722) (0.0299,0.6756) (0.0300,0.6789) (0.0300,0.6823) (0.0300,0.6856) (0.0301,0.6890) (0.0301,0.6923) (0.0302,0.6957) (0.0304,0.6990) (0.0304,0.7023) (0.0304,0.7057) (0.0304,0.7090) (0.0305,0.7124) (0.0305,0.7157) (0.0306,0.7191) (0.0308,0.7224) (0.0309,0.7258) (0.0310,0.7291) (0.0310,0.7324) (0.0311,0.7358) (0.0312,0.7391) (0.0313,0.7425) (0.0313,0.7458) (0.0314,0.7492) (0.0314,0.7525) (0.0316,0.7559) (0.0316,0.7592) (0.0316,0.7625) (0.0318,0.7659) (0.0318,0.7692) (0.0319,0.7726) (0.0322,0.7759) (0.0322,0.7793) (0.0323,0.7826) (0.0325,0.7860) (0.0326,0.7893) (0.0326,0.7926) (0.0327,0.7960) (0.0329,0.7993) (0.0330,0.8027) (0.0331,0.8060) (0.0333,0.8094) (0.0333,0.8127) (0.0333,0.8161) (0.0333,0.8194) (0.0334,0.8227) (0.0335,0.8261) (0.0337,0.8294) (0.0337,0.8328) (0.0339,0.8361) (0.0342,0.8395) (0.0344,0.8428) (0.0344,0.8462) (0.0344,0.8495) (0.0345,0.8528) (0.0345,0.8562) (0.0346,0.8595) (0.0347,0.8629) (0.0348,0.8662) (0.0349,0.8696) (0.0352,0.8729) (0.0352,0.8763) (0.0353,0.8796) (0.0354,0.8829) (0.0356,0.8863) (0.0359,0.8896) (0.0359,0.8930) (0.0360,0.8963) (0.0362,0.8997) (0.0363,0.9030) (0.0364,0.9064) (0.0365,0.9097) (0.0366,0.9130) (0.0368,0.9164) (0.0369,0.9197) (0.0369,0.9231) (0.0369,0.9264) (0.0369,0.9298) (0.0372,0.9331) (0.0372,0.9365) (0.0378,0.9398) (0.0379,0.9431) (0.0380,0.9465) (0.0382,0.9498) (0.0384,0.9532) (0.0385,0.9565) (0.0386,0.9599) (0.0387,0.9632) (0.0387,0.9666) (0.0389,0.9699) (0.0392,0.9732) (0.0394,0.9766) (0.0418,0.9799) (0.0420,0.9833) (0.0424,0.9866) (0.0441,0.9900) (0.0447,0.9933) (0.0475,0.9967) (0.0492,1.0000) };
\addlegendentry{NU Campus (DL)}
% Data for Fenway Park (DL)
\addplot+[mark=none] coordinates {%
(0.0502,0.0204) (0.0506,0.0408) (0.0521,0.0612) (0.0546,0.0816) (0.0558,0.1020) (0.0577,0.1224) (0.0580,0.1429) (0.0589,0.1633) (0.0599,0.1837) (0.0604,0.2041) (0.0604,0.2245) (0.0606,0.2449) (0.0607,0.2653) (0.0607,0.2857) (0.0609,0.3061) (0.0612,0.3265) (0.0614,0.3469) (0.0621,0.3673) (0.0622,0.3878) (0.0622,0.4082) (0.0622,0.4286) (0.0623,0.4490) (0.0630,0.4694) (0.0631,0.4898) (0.0632,0.5102) (0.0634,0.5306) (0.0635,0.5510) (0.0636,0.5714) (0.0643,0.5918) (0.0645,0.6122) (0.0646,0.6327) (0.0646,0.6531) (0.0648,0.6735) (0.0649,0.6939) (0.0652,0.7143) (0.0655,0.7347) (0.0658,0.7551) (0.0663,0.7755) (0.0663,0.7959) (0.0664,0.8163) (0.0664,0.8367) (0.0667,0.8571) (0.0667,0.8776) (0.0669,0.8980) (0.0671,0.9184) (0.0682,0.9388) (0.0689,0.9592) (0.0692,0.9796) (0.0717,1.0000) };
\addlegendentry{Fenway Park (DL)}
% Data for NU Campus (EST)
\addplot+[mark=none] coordinates {%
(0.3018,0.0033) (0.3097,0.0067) (0.3120,0.0100) (0.3124,0.0134) (0.3142,0.0167) (0.3152,0.0201) (0.3170,0.0234) (0.3178,0.0268) (0.3205,0.0301) (0.3223,0.0334) (0.3256,0.0368) (0.3297,0.0401) (0.3338,0.0435) (0.3338,0.0468) (0.3368,0.0502) (0.3370,0.0535) (0.3374,0.0569) (0.3377,0.0602) (0.3383,0.0635) (0.3384,0.0669) (0.3399,0.0702) (0.3403,0.0736) (0.3406,0.0769) (0.3407,0.0803) (0.3417,0.0836) (0.3424,0.0870) (0.3431,0.0903) (0.3434,0.0936) (0.3434,0.0970) (0.3439,0.1003) (0.3439,0.1037) (0.3440,0.1070) (0.3440,0.1104) (0.3443,0.1137) (0.3450,0.1171) (0.3453,0.1204) (0.3457,0.1237) (0.3457,0.1271) (0.3462,0.1304) (0.3463,0.1338) (0.3469,0.1371) (0.3469,0.1405) (0.3474,0.1438) (0.3476,0.1472) (0.3481,0.1505) (0.3483,0.1538) (0.3489,0.1572) (0.3503,0.1605) (0.3517,0.1639) (0.3518,0.1672) (0.3520,0.1706) (0.3529,0.1739) (0.3533,0.1773) (0.3541,0.1806) (0.3545,0.1839) (0.3554,0.1873) (0.3554,0.1906) (0.3559,0.1940) (0.3566,0.1973) (0.3579,0.2007) (0.3585,0.2040) (0.3587,0.2074) (0.3597,0.2107) (0.3610,0.2140) (0.3625,0.2174) (0.3627,0.2207) (0.3629,0.2241) (0.3630,0.2274) (0.3640,0.2308) (0.3644,0.2341) (0.3651,0.2375) (0.3652,0.2408) (0.3655,0.2441) (0.3666,0.2475) (0.3670,0.2508) (0.3674,0.2542) (0.3689,0.2575) (0.3690,0.2609) (0.3692,0.2642) (0.3699,0.2676) (0.3702,0.2709) (0.3710,0.2742) (0.3710,0.2776) (0.3723,0.2809) (0.3731,0.2843) (0.3741,0.2876) (0.3743,0.2910) (0.3744,0.2943) (0.3754,0.2977) (0.3755,0.3010) (0.3756,0.3043) (0.3757,0.3077) (0.3761,0.3110) (0.3762,0.3144) (0.3762,0.3177) (0.3766,0.3211) (0.3767,0.3244) (0.3784,0.3278) (0.3784,0.3311) (0.3786,0.3344) (0.3789,0.3378) (0.3794,0.3411) (0.3799,0.3445) (0.3799,0.3478) (0.3806,0.3512) (0.3809,0.3545) (0.3816,0.3579) (0.3820,0.3612) (0.3827,0.3645) (0.3829,0.3679) (0.3829,0.3712) (0.3833,0.3746) (0.3840,0.3779) (0.3842,0.3813) (0.3844,0.3846) (0.3844,0.3880) (0.3846,0.3913) (0.3846,0.3946) (0.3858,0.3980) (0.3861,0.4013) (0.3867,0.4047) (0.3867,0.4080) (0.3871,0.4114) (0.3873,0.4147) (0.3879,0.4181) (0.3881,0.4214) (0.3882,0.4247) (0.3882,0.4281) (0.3889,0.4314) (0.3893,0.4348) (0.3893,0.4381) (0.3930,0.4415) (0.3952,0.4448) (0.3979,0.4482) (0.3999,0.4515) (0.4016,0.4548) (0.4017,0.4582) (0.4040,0.4615) (0.4081,0.4649) (0.4091,0.4682) (0.4094,0.4716) (0.4094,0.4749) (0.4097,0.4783) (0.4116,0.4816) (0.4119,0.4849) (0.4126,0.4883) (0.4127,0.4916) (0.4140,0.4950) (0.4140,0.4983) (0.4146,0.5017) (0.4568,0.5050) (0.4594,0.5084) (0.4616,0.5117) (0.4623,0.5151) (0.4703,0.5184) (0.4747,0.5217) (0.4761,0.5251) (0.4763,0.5284) (0.4764,0.5318) (0.4767,0.5351) (0.4768,0.5385) (0.4768,0.5418) (0.4788,0.5452) (0.4790,0.5485) (0.4792,0.5518) (0.4807,0.5552) (0.4809,0.5585) (0.4825,0.5619) (0.4827,0.5652) (0.4831,0.5686) (0.4833,0.5719) (0.4839,0.5753) (0.4844,0.5786) (0.4845,0.5819) (0.4847,0.5853) (0.4849,0.5886) (0.4850,0.5920) (0.4857,0.5953) (0.4858,0.5987) (0.4872,0.6020) (0.4895,0.6054) (0.4898,0.6087) (0.4898,0.6120) (0.4916,0.6154) (0.4918,0.6187) (0.4918,0.6221) (0.4918,0.6254) (0.4944,0.6288) (0.4945,0.6321) (0.4960,0.6355) (0.4961,0.6388) (0.4961,0.6421) (0.4962,0.6455) (0.4973,0.6488) (0.4997,0.6522) (0.5000,0.6555) (0.5012,0.6589) (0.5020,0.6622) (0.5031,0.6656) (0.5046,0.6689) (0.5070,0.6722) (0.5081,0.6756) (0.5091,0.6789) (0.5114,0.6823) (0.5115,0.6856) (0.5122,0.6890) (0.5131,0.6923) (0.5132,0.6957) (0.5134,0.6990) (0.5143,0.7023) (0.5145,0.7057) (0.5148,0.7090) (0.5151,0.7124) (0.5158,0.7157) (0.5159,0.7191) (0.5172,0.7224) (0.5182,0.7258) (0.5184,0.7291) (0.5197,0.7324) (0.5198,0.7358) (0.5201,0.7391) (0.5215,0.7425) (0.5216,0.7458) (0.5239,0.7492) (0.5243,0.7525) (0.5246,0.7559) (0.5261,0.7592) (0.5261,0.7625) (0.5276,0.7659) (0.5293,0.7692) (0.5322,0.7726) (0.5327,0.7759) (0.5334,0.7793) (0.5335,0.7826) (0.5336,0.7860) (0.5348,0.7893) (0.5377,0.7926) (0.5382,0.7960) (0.5388,0.7993) (0.5392,0.8027) (0.5393,0.8060) (0.5394,0.8094) (0.5403,0.8127) (0.5404,0.8161) (0.5418,0.8194) (0.5424,0.8227) (0.5426,0.8261) (0.5450,0.8294) (0.5458,0.8328) (0.5459,0.8361) (0.5460,0.8395) (0.5460,0.8428) (0.5477,0.8462) (0.5477,0.8495) (0.5482,0.8528) (0.5483,0.8562) (0.5486,0.8595) (0.5503,0.8629) (0.5503,0.8662) (0.5504,0.8696) (0.5512,0.8729) (0.5514,0.8763) (0.5516,0.8796) (0.5520,0.8829) (0.5542,0.8863) (0.5548,0.8896) (0.5549,0.8930) (0.5549,0.8963) (0.5550,0.8997) (0.5550,0.9030) (0.5551,0.9064) (0.5587,0.9097) (0.5587,0.9130) (0.5592,0.9164) (0.5597,0.9197) (0.5597,0.9231) (0.5604,0.9264) (0.5604,0.9298) (0.5606,0.9331) (0.5610,0.9365) (0.5610,0.9398) (0.5612,0.9431) (0.5615,0.9465) (0.5628,0.9498) (0.5630,0.9532) (0.5633,0.9565) (0.5633,0.9599) (0.5637,0.9632) (0.5648,0.9666) (0.5649,0.9699) (0.5652,0.9732) (0.5667,0.9766) (0.5676,0.9799) (0.5685,0.9833) (0.5698,0.9866) (0.5726,0.9900) (0.5727,0.9933) (0.5737,0.9967) (0.5778,1.0000) };
\addlegendentry{NU Campus (EST)}
% Data for Fenway Park (EST)
\addplot+[mark=none] coordinates {%
(0.0712,0.0204) (0.0723,0.0408) (0.0726,0.0612) (0.0728,0.0816) (0.0732,0.1020) (0.0732,0.1224) (0.0733,0.1429) (0.0735,0.1633) (0.0738,0.1837) (0.0741,0.2041) (0.0745,0.2245) (0.0755,0.2449) (0.0759,0.2653) (0.0778,0.2857) (0.0785,0.3061) (0.0790,0.3265) (0.0816,0.3469) (0.0825,0.3673) (0.0852,0.3878) (0.0858,0.4082) (0.0859,0.4286) (0.0869,0.4490) (0.0875,0.4694) (0.0879,0.4898) (0.0880,0.5102) (0.0904,0.5306) (0.1472,0.5510) (0.1773,0.5714) (0.1845,0.5918) (0.1936,0.6122) (0.1964,0.6327) (0.2010,0.6531) (0.2012,0.6735) (0.2033,0.6939) (0.2045,0.7143) (0.2059,0.7347) (0.2131,0.7551) (0.2138,0.7755) (0.2142,0.7959) (0.2198,0.8163) (0.2215,0.8367) (0.2247,0.8571) (0.2255,0.8776) (0.2271,0.8980) (0.2295,0.9184) (0.2410,0.9388) (0.2430,0.9592) (0.2447,0.9796) (0.2535,1.0000) };
\addlegendentry{Fenway Park (EST)}


==> figures/ecdf_meas_data.tex <==
% Data for Calibrated
\addplot+[mark=none] coordinates {%
(0.0039,0.0204) (0.0041,0.0408) (0.0041,0.0612) (0.0043,0.0816) (0.0044,0.1020) (0.0047,0.1224) (0.0048,0.1429) (0.0049,0.1633) (0.0056,0.1837) (0.0056,0.2041) (0.0060,0.2245) (0.0065,0.2449) (0.0067,0.2653) (0.0075,0.2857) (0.0080,0.3061) (0.0081,0.3265) (0.0081,0.3469) (0.0089,0.3673) (0.0090,0.3878) (0.0091,0.4082) (0.0099,0.4286) (0.0106,0.4490) (0.0107,0.4694) (0.0113,0.4898) (0.0113,0.5102) (0.0114,0.5306) (0.0115,0.5510) (0.0117,0.5714) (0.0118,0.5918) (0.0119,0.6122) (0.0124,0.6327) (0.0132,0.6531) (0.0133,0.6735) (0.0135,0.6939) (0.0136,0.7143) (0.0144,0.7347) (0.0159,0.7551) (0.0168,0.7755) (0.0174,0.7959) (0.0175,0.8163) (0.0184,0.8367) (0.0190,0.8571) (0.0201,0.8776) (0.0234,0.8980) (0.0255,0.9184) (0.0479,0.9388) (0.0481,0.9592) (0.0486,0.9796) (0.0565,1.0000) };
\addlegendentry{Calibrated}
% Data for Uncalibrated
\addplot+[mark=none] coordinates {%
(0.0045,0.0204) (0.0045,0.0408) (0.0049,0.0612) (0.0059,0.0816) (0.0291,0.1020) (0.0313,0.1224) (0.0348,0.1429) (0.0353,0.1633) (0.0353,0.1837) (0.0354,0.2041) (0.0371,0.2245) (0.0390,0.2449) (0.0391,0.2653) (0.0398,0.2857) (0.0432,0.3061) (0.0433,0.3265) (0.0447,0.3469) (0.0473,0.3673) (0.0492,0.3878) (0.0502,0.4082) (0.0532,0.4286) (0.0535,0.4490) (0.0556,0.4694) (0.0559,0.4898) (0.0569,0.5102) (0.0584,0.5306) (0.0590,0.5510) (0.0591,0.5714) (0.0606,0.5918) (0.0607,0.6122) (0.0612,0.6327) (0.0612,0.6531) (0.0613,0.6735) (0.0614,0.6939) (0.0614,0.7143) (0.0629,0.7347) (0.0636,0.7551) (0.0641,0.7755) (0.0645,0.7959) (0.0648,0.8163) (0.0650,0.8367) (0.0659,0.8571) (0.0662,0.8776) (0.0666,0.8980) (0.0667,0.9184) (0.0669,0.9388) (0.0681,0.9592) (0.0709,0.9796) (0.0774,1.0000) };
\addlegendentry{Uncalibrated}

